Algorithms for Fair Team Formation in Online Labour Marketplaces

As freelancing work keeps on growing almost everywhere due to a sharp decrease in communication costs and to the widespread of Internet-based labour marketplaces (e.g., guru.com, feelancer.com, mturk.com, upwork.com), many researchers and practitioners have started exploring the benefits of outsourcing and crowdsourcing. Since employers often use these platforms to find a group of workers to complete a specific task, researchers have focused their efforts on the study of team formation and matching algorithms and on the design of effective incentive schemes. Nevertheless, just recently, several concerns have been raised on possibly unfair biases introduced through the algorithms used to carry out these selection and matching procedures. For this reason, researchers have started studying the fairness of algorithms related to these online marketplaces, looking for intelligent ways to overcome the algorithmic bias that frequently arises. Broadly speaking, the aim is to guarantee that, for example, the process of hiring workers through the use of machine learning and algorithmic data analysis tools does not discriminate, even unintentionally, on grounds of nationality or gender. In this short paper, we define the Fair Team Formation problem in the following way: given an online labour marketplace where each worker possesses one or more skills, and where all workers are divided into two or more not overlapping classes (for examples, men and women), we want to design an algorithm that is able to find a team with all the skills needed to complete a given task, and that has the same number of people from all classes. We provide inapproximability results for the Fair Team Formation problem together with four algorithms for the problem itself. We also tested the effectiveness of our algorithmic solutions by performing experiments using real data from an online labor marketplace.

==> experiments-removed.tex <==


\note[ChaTo]{
Bring some material commented in section 4.3 to the experiments, indicate the submission 

Explain how we set $\alpha$ in the experiments. That we use $\alpha=4$ experimentally, we tried $\alpha = 1 \dots 20$. The effect of different $\alpha$s is to make TFO behave more differently from always-outsource. We also selected $k=15$, we tried $k = 1 \dots 20$.}

\note[Adri]{Now, the following is totally out of context.}
The key difference that one can observe between the first
two plots and the last two is in
the relative performance of \algoAlwaysOutsource when compared to
{\naivetfo} and {\algowithsalary}.  When $x=0.02$
%$\salary{r}=0.02\outsourcecost{r}$ 
(i.e., the outsource cost per task is $50$
times larger than the salary cost of a worker per unit of time), then
\algoAlwaysOutsource performs significantly worse than both {\naivetfo} and
{\algowithsalary}; this is evident in Figures~\ref{d1:smallsalary},
\ref{d2:smallsalary}. % and \ref{d3:smallsalary}.
On the other hand,
when $x=0.1$ and 
{$\salary{r}=0.1\outsourcecost{r}$} 
(i.e., the outsource cost of a
worker is just $10$ times larger than his salary), then
\algoAlwaysOutsource performs better than {\algowithsalary}; this is
shown in Figures~\ref{d1:largesalary} and~\ref{d2:largesalary}.  It is worth noting that in this case the
heuristic algorithm {\naivetfo} performs almost as good as
\algoAlwaysOutsource and outperforms the theoretically-justified
{\algowithsalary} algorithm.

\spara{Exploring the limits of the {\algowithsalary} algorithm:}
Our experiments for the {\problemsalary} problem
demonstrate that the relative performance of
{\algowithsalary} compared to \algoAlwaysOutsource depends on two
factors: $(1)$ the 
salary-to-outsource ratio $x$ 
and $(2)$ the coherence parameter of the workload $p$.
Whereas in our previous experiments we have set reasonable values for these parameters, we
want to study further the behavior of the \algowithsalary algorithm. Namely, we want to investigate for
what values of these parameters it outperforms and for what it is
outperformed by \algoAlwaysOutsource. Thus, we have performed
experiments by generating workload streams varying both $x$ and~$p$
%$(x, p)\in\{0.01,0.02,\ldots 0.1\}$.
%
%
%Although $(1)$ has been hinted by the set of results shown in
%Figure~\ref{fig:results-problem-salary}, exploring $(2)$ requires some
%further experimentation. 
%For this, we 
%generate data using different values of the coherence parameter $p\in\{0.01,0.02,\ldots 0.1\}$.


Figure~\ref{fig:exp-local-details} shows the ratio of the cost
achieved by \algowithsalary over the cost achieved by the
\algoAlwaysOutsource heuristic; the smaller this value the better the
performance of \algowithsalary compared to \algoAlwaysOutsource.
Each cell in the heatmap corresponds to a specific problem setting, as
defined by the values of the $(x,p)$-pair. (Here as well, the value of
each cell is the average of 100 runs on different workload streams.)
The results for 
the UpWork (Figure~\ref{fig:upwork-exploration}), 
the Freelancer (Figure~\ref{fig:freelancer-exploration}) and the Guru
(Figure~\ref{fig:guru-exploration}) datasets
show how we can nicely characterize the border in the parameter
space between the areas where  
\algowithsalary is better than
\algoAlwaysOutsource and where it is worse. The results 
demonstrate that the smaller the value of $x$ and $p$ the better the performance
of \algowithsalary compared to \algoAlwaysOutsource. As one can
expect, this means that
in settings for which the salary is high compared to the outsourcing cost, and
in settings for which there is high variability in (consecutive) tasks that
are needed to be executed, outsourcing is economically advantageous and hiring
permanent workers may be an overkill.

We have also compared the behavior of \naivetfo with
\algoAlwaysOutsource. The results are similar, actually somewhat better
(the border is shifted slightly up and to the right), and we omit them
from the paper.
\note[Adri]{We should do that now with the new settings.}

\note[ChaTo]{We have also done experiments varying hiring cost $\hiringcost{r}$ from $1\outsourcecost{r}$ to $16\outsourcecost{r}$}

\iffalse
\spara{Experiments with high task locality:}
We note that in general the simple \algoAlwaysOutsource strategy
performs the best across all datasets. This is because of the diversity
of workers and tasks in each platform, which does not make it economical
to hire anyone.
%
Instead, in this section we produce a stream of tasks for D1 and D2 in
which the tasks change {\em locally}, i.e., a task is more likely to be
similar to the next task than if we were sampling at random.

In order to achieve this, we run the following procedure:

\begin{enumerate}
\item Pick a random task as a pivot.
\item With probability $1-p$, pick the next task within those that are
similar enough to the pivot, i.e., those whose Jaccard similarity with
the pivot is larger than a threshold $\theta$.
\item With probability $p$, pick another random task as a pivot.
\end{enumerate}
\fi


%\begin{figure}[t]
%\subfigure[Freelancer $p=0.1$]{\includegraphics[width=.23\textwidth]{fig/salary/local_streams/Local_Salary_Freelancer_ThJacc05_JP01_MinCluSize_2.eps}}
%\subfigure[Freelancer $p=0.01$]{\includegraphics[width=.23\textwidth]{fig/salary/local_streams/Local_Salary_Freelancer_ThJacc05_JP001_MinCluSize_2.eps}}
%
%\centering\subfigure[Guru $p=0.1$]{\includegraphics[width=.23\textwidth]{fig/salary/local_streams/Local_Salary_Guru_ThJacc05_JP01_MinCluSize_2.eps}}
%\subfigure[Guru $p=0.01$]{\includegraphics[width=.23\textwidth]{fig/salary/local_streams/Local_Salary_Guru_ThJacc05_JP001_MinCluSize_2.eps}}
%
%\caption{Results obtained using a stream of tasks with task locality, selecting tasks that are similar to the current pivot with probability $1-p$, and selecting another pivot with probability $p$. In all cases, the similarity threshold is $\theta=0.5$.}
%\label{fig:exp-local-details}
%\end{figure}

%\begin{figure}[t]
%\subfigure[Freelancer]{\includegraphics[width=.235\textwidth]{fig/salary/local_streams/heat_maps/heat_map_VS_Always_Outsource__FREELANCER__K15.eps}\label{fig:freelancer-exploration}}
%\subfigure[Guru]{\includegraphics[width=.235\textwidth]{fig/salary/local_streams/heat_maps/heat_map_VS_Always_Outsource__GURU__K15.eps}\label{fig:guru-exploration}}
%
%\caption{Ratio of the cost achieved by \algowithsalary and
%  \algoAlwaysOutsource after 10K tasks for various %combinations of the
%    coherence parameter $p$ and the salary-to-outsource ratio %$x$. Colors
%    represent the ratio of costs: blue indicates the region %where
%    \algowithsalary has smaller cost, red the region where
%    \algoAlwaysOutsource has smaller cost, and white the %region where they are equivalent. The
%    region where \algowithsalary is better is characterized by %high workload
%    coherence (small $p$) and small salary-to-outsource ratio %(i.e.,
%	smaller salaries).
%%Experiments for the Freelancer and Guru datasets using different values
%%of the coherence parameter $p\in \{0.01, 0.02,\dots, 0.1\}$ and the
%%salary-to-outsource ratio $x\in\{0.01,0.02,\ldots ,0.1\}$. The colours
%%in the cells represent the ratio of the cost of achieved by
%%{\algowithsalary} over \algoAlwaysOutsource.
%}
%\label{fig:exp-local-details}
%\end{figure}


\iffalse

We considered a pivot as eligible only if it had at least one other task
that was similar enough to it. We experimented with various values of
$p$ and $\theta$. Figure~\ref{fig:exp-local-details} shows results for
$\theta=0.5$, $p=0.1, 0.01$.
%
In general, we observe that with a smaller value of $p$, which yields
longer subsequences of tasks similar to a pivot, generates a workload in
which hiring becomes more efficient than outsourcing.
\fi


==> related.tex <==

To the best of our knowledge, 
we are the first to introduce and solve the Fair Team Formation problem.
However, our work is related to existing work on crowdsourcing, team formation, and fairness, which we outline next.

\spara{Crowdsourcing.}
Among the extensive literature in crowdsourcing, probably the most related to ours is the work of 
\citet{ho2012online}. Their goal is to assign individual workers to 
tasks, based on the workers' skills.
Although Ho and Vaughan also deploy the primal--dual 
technique
in order to solve the task-assignment problem,
the tasks they consider
can be performed by individual workers and not by teams. As a result, both their problem and 
their algorithm is different from ours. 
%Moreover, their main goal is to learn the skills of the individuals from past tasks. This problem is orthogonal to our work, as we assume that the workers' skills are part of the input. 
 
\spara{Team formation.} 
A large body of work in team formation considers the following problem: given a social or a collaboration
network among the workers and a set of 
skills that needed to be covered, select a team of experts that can collectively cover all the required skills, while minimizing the communication cost
between the team members~\cite{anagnostopoulos12online, an13finding,dorn10composing,gajewar12multiskill,kargar11teamexp,lappas2009finding,li10team,sozio10community}.
Other variants of this problem have also considered
optimizing the cost of recruiting promising candidates for a set of pre-defined tasks in an offline fashion~\cite{golshan14profit} and minimizing the workload assigned to
each individual team member~\cite{majumder12capacitated,anagnostopoulos2010power}. %identifying effective leaders~\cite{kargar11teamexp}, or optimizing the individual's benefit from team participation~\cite{agrawal14grouping}.

Although the concept of set-cover is common between our work and previous work,
the framework we propose on this paper is different in multiple dimensions.
%
First,  we do not focus on optimizing the communication cost; 
in fact we do not assume any network among the individual workers. Our goal is to minimize
the overall cost paid on hiring, outsourcing, and salary costs. 
%
This difference in the objectives leads to different
(and new) optimization problems that we need to solve.
%
Secondly, most of the work above focuses on the offline version
of the team-formation problem, where the tasks to be completed are 
a-priori known to the algorithm. The exception is the work of \citet{anagnostopoulos2010power,anagnostopoulos12online}. %, 
%who consider the online setting where jobs arrive one-at-a-time and their characteristics are not known to the algorithm in advance.
%
 However, in their setting they aim to distribute the workload as evenly as possible among the workers,
while our objective is to minimize the overall cost of maintaining a team that can complete the 
arriving tasks. 
Moreover, the option of outsourcing that we propose is new with respect to the team formation literature. Finally, in the design
of our online algorithms we use the primal--dual framework, which was not the case for previous work on online team formation.

\spara{Fairness.}






==> salarynew-proofs.tex <==
In this section we provide some details missing from
Section~\ref{sec:salarynew}, as well as proofs for the mathematical
resuts.

Throughout this section, we use $[a,b]$ to denote the time interval  $[a, a+1, \dots, b]$.


%
%The setting we consider in this section is similar 
%to the one we considered in the previous section
%every worker $\worker{r}$ is associated with 
%a hiring cost $\hiringcost{r}$, which is a lump sum paid when the worker is hired and
%an outsource cost $\outsourcecost{r}$, which is paid every time
%$\worker{r}$ is outsourced.
%In addition to that, the new feature of {\problemsalary} is that every
%worker $\worker{r}$ who is hired
%is paid a salary 
%$\salary{r}$ for every unit of time he is employed.
%In this version of the problem, workers can be hired and then fired and therefore, 
%in this setting the hiring cost $\hiringcost{r}$ can be viewed as the signup bonus
%of a worker (or the severance package when fired).
%
%\spara{The linear program:} 
%The linear program that describes the \problemsalary problem can be formulated similarly
%to the one we formed for \problemuseforfree.  
%
%A key notion that is new in this linear problem is the notion of intervals 
%defined by a worker $\worker{r}$, denoted by $\intervals$.
%These are the time 
%intervals for which $\worker{r}$ was hired.
%The underlying assumption in the definition of these intervals is that 
%at every time-unit a new task arrives.
%Given these intervals $\intervals$ for every worker $\worker{r}$, we also introduce variable
%$x(r,I)$ such that for $I\in \intervals$, $x(r,I)=1$ if worker
%$\worker{r}$ is hired during the entire interval $I$;
%otherwise $x(r,I)=0$.
%
%We also introduce variable $g_{rt}$ such that 
%$g_{rt}=1$ if worker $\worker{r}$ receives salary at time $t$; otherwise
%$g_{rt}=0$. Note that $\worker{r}$ receives salary if and only if
%$\worker{r}$ is hired.
%
%
%Given the above we can formulate the following linear program for the {\problemsalary} problem:
%
%\begin{framed}
%Linear program for {\problemsalary}:
%\[
%\min \sum_{r = 1}^{\numworkers} \left[ \sum_{I\in \intervals}  \hiringcost{r} x(r,I)
% + \sum_{t=1}^{\numtasks} \outsourcecost{r}  f_{rt} +  \sum_{t=1}^{\numtasks} \salary{r}  g_{rt} \right]
%\]
%subject to\\
%$\forall t=1\ldots\numtasks, \ell\in\task{t}:$
%\begin{eqnarray}
%\label{eq:cover-skills-original}
%\sum_{r\in P_\ell}\left(f_{rt} + \sum_{I\in \intervals: t\in I} x(r,I) \right) &\geq& 1.
%\end{eqnarray}
%$\forall t=1\ldots\numtasks, r=1\ldots\numworkers:$
%\begin{eqnarray}
%\label{eq:salary-constraint}
%\sum_{I\in \intervals: t\in I}  x(r,I) \leq g_{rt}
%\end{eqnarray}
%$\forall t=1\ldots\numtasks, r=1\ldots\numworkers,I\in\intervals:$
%\[x(r,I), f_{rt}, g_{rt}\ge0\]
%\end{framed}
%\medskip
%
%
%
%It turns out to be hard to design an approximation algorithm using
%directly this program, the main reason being that it is hard to keep track of the costs being paid
%for every worker when the intervals of him being hired, outsourced and idle are of variable length. 
%Therefore, we will resort to a different approach:
%We will consider an \emph{alternative problem}, by formulating an \emph{alternative
%linear program}. We call this problem the {\problemalternative} problem.
%In this alternative problem, we will restrict our solution to consider for each worker intervals of fixed length.
%However, any solution to {\problemalternative}, and its corresponding linear program, will also be
%a feasible solution to the {\problemsalary}.
%
%\spara{Overall strategy:} Therefore, our overall strategy is the following:
%$(i)$ First, we will  present a
%linear-programming formulation for the {\problemalternative} problem, and its
%dual. $(ii)$ Based on these linear programs we will design an algorithm for
%the {\problemalternative} problem. $(iii)$ Then, we will prove an approximation ratio
%between the produced solution and the optimal solution for the {\problemalternative} problem. 
%$(iv)$ Finally, we will prove that any solution of the
%{\problemsalary} problem
%can be transformed to a feasible solution 
%of the {\problemalternative} problem
%that is only a factor of at most $3$ times higher.
%This, in particular holds for the optimal solution of {\problemsalary}.
%This implies that the optimal solution to  {\problemalternative} 
%is at most a factor 3 worse of the optimal solution of the
%original problem.
%
%
%\subsection{The {\problemalternative} problem}
%This alternative problem formulation and corresponding linear program will restrict 
%the solutions to have a specific structure; 
%whenever a worker $\worker{r}$ is hired he is
%then fired after $\hireintervals_r\Def \Ceil{\hiringcost{r}/\salary{r}}$ time
%units---independently of whether he is used or not in tasks within these $\hireintervals_r$ time units.
%
%The combined hiring and salary cost of worker $\worker{r}$  then includes both
%the hiring cost $\hiringcost{r}$ and the salary paid for $\hireintervals_r$ time
%units. This combined cost for time units $\hireintervals_r$ is bounded  by
%$\hiringcost{r}+\hireintervals_r\cdot\salary{r}\le (2 +
%    \salary{r}/\hiringcost{r}) \cdot\hiringcost{r} \leq 3 \hiringcost{r} $.
%Therefore, throughout we will use: 
%$\hiringcostwithsalary{r}\Def 3 \cdot\hiringcost{r}$.
%
%A solution to the alternative linear program,  will also be a feasible solution to our original
%problem (by setting also $g_{rt}=1$ for each $r, t\in I$ for which
%$x(r,I)=1$, and 0 otherwise). The question is  whether there exists a good solution with
%this specific structure that is also a good solution to the original
%problem. We answer affirmatively this question  by showing that any
%solution for the original problem can be turned into a feasible solution
%for this linear program at the expenses of a small loss in the
%approximation factor.
%
%We start by defining the linear program for the {\problemalternative}.
%For each worker $\worker{r}$, we denote
%by $\intervals$ the set of intervals for which worker $\worker{r}$ was hired.
%Recall that all these intervals are of fixed length $\hireintervals_r$. The generic such interval that starts at time $t$
%is also denoted by $I_r^t$.
%A worker $\worker{r}$ has $x(r,I) = 1$ if and only if the worker is hired during
%the \emph{entire} interval $I$. 
%
%The linear program that corresponds to this alternative problem formulation is the following:
%
%\begin{framed}
%Linear program for {\problemalternative}:
%\[
%\min \sum_{r = 1}^{\numworkers} \left[ \sum_{I\in \intervals}  \hiringcostwithsalary{r} x(r,I)
% + \sum_{t=1}^{\numtasks} \outsourcecost{r}  f_{rt} \right]
%\]
%subject to\\
%$\forall t=1\ldots\numtasks, \ell\in\task{t}:$
%\begin{eqnarray}
%\label{eq:cover-skills-alt}
%\sum_{r\in P_\ell}\left(f_{rt} + \sum_{I\in \intervals: t\in I} x(r,I) \right) &\geq& 1.
%\end{eqnarray}
%$\forall t=1\ldots\numtasks, r=1\ldots\numworkers,I\in\intervals:$
%\[x(r,I), f_{rt}\ge0\]
%\end{framed}
%\medskip

\subsection{Conversion of solution to \problemalternative to a solution to
  \problemsalary}

In Section~\ref{subsec:alt-to-salary} we describe the algorithm
\algowithsalary. It creates a solution to the LP
for \problemsalary by taking the solution produced by \altalgo, which is
feasible for the LP of \problemalternative, using the same variable
values, and in addition setting $g_{rt}=1$ for each $r, t\in I$ for which
$x(r,I)=1$, and $g_{rt}=0$ otherwise. In Lemma~\ref{lemma:altTFOToTFO}
we prove that the solution produced is feasible and we bound its
expected cost.


A small technical note is necessary here. Note that both linear prograns 
(for \problemsalary and for \problemalternative) allow for solutions in which for a worker
$\worker{r}$ two overlapping intervals have $x(r,I_1)=x(r,I_2)=1$. For
\problemalternative, because
intervals have length exactly $\hireintervals_r$, this may happen even in the optimal
solution---consider, for instance, if for a worker $\worker{r}$ we have that
$T=2\hireintervals_r-1$, then the optimal solution may decide to always hire worker
$\worker{r}$, leading to two different intervals $I_1,I_2$ having $x(r,I_1)=x(r,I_2)=1$.
Nevertheless, such a solution, when transformed to a solution for
\problemsalary, it can be further transformed to a solution with no higher
cost, in which this does not happen. In any case, in the proof of Lemma
\ref{lemma:altTFOToTFO}, we show that the \algowithsalary algorithm creates solutions in which this does not happen, in
other words, for each worker $\worker{r}$, there are no overlapping
intervals $I_1, I_2, I_1\ne I_2$, in which $I_1\cap I_2 \ne \emptyset$ and
$x(r,I_1) = x(r, I_2) = 1$.

%The dual of the above alternative program is the following:
%
%\medskip
%\begin{framed}
%The dual of the linear program for {\problemalternative}:
%\[
%\max \sum_{t=1}^T
% \sum_{\ell\in\task{t}} u_{\ell t} 
%\]
%subject to:\\ 
%$\forall r=1\ldots\numworkers, I\in\intervals$:
%\begin{eqnarray}\label{eq:salary-alt-evict}
% \sum_{t\in I} \sum_{\ell\in\task{t}\cap\worker{r}} u_{lt}
% & \leq & \hiringcostwithsalary{r} 
%\end{eqnarray}
%$\forall t=1\ldots\numtasks, r=1\ldots\numworkers$:
%\begin{eqnarray}\label{eq:salary-alt-outsource}
%\sum_{\ell\in\task{t}\cap\worker{r}}u_{\ell t} &\leq &\outsourcecost{r}
%\end{eqnarray}
%$\forall \ell\in\task{t},  t=1\ldots\numtasks$:
%\[u_{\ell t}\ge0\]
%\end{framed}
%\medskip
%
%\subsection{Algorithm}
%In this section we first present an algorithm for the {\problemalternative}
%and we then show how to transform its solution to a solution for the original {\problemsalary}
%problem.
%
%\spara{The algorithm for} {\problemalternative}:
%Our algorithm for {\problemalternative}, 
%which we call {\altalgo},
%is based on the {\problemalternative} linear program 
%given above.  
%
%Similarly to Section~\ref{sec:useforfree}, we define
%%\[\rho_2_t=\ln\numworkers+\ln\maxhiringcost{r}+2\ln t+\ln 3\,\]
%\[\rho_2=\ln\numworkers+\ln\maxhiringcostwithsalary{r}+\ln\numtasksTotal,\]
%where
%$\maxhiringcostwithsalary{r}=\max_{r\in\workerset}\hiringcostwithsalary{r}$.
%and recall that $\numtasksTotal$ is the total number of tasks that
%will arrive (or we can use an upper bound on that value, that we assume
%that we know).
%
%
%\begin{enumerate}
%
%\item Let $\nonhiredworkers^\numtasks$ and $\hiredworkers^\numtasks$ represent the
%workers that are not hired and hired, respectively, at the time that
%$\task{\numtasks}$ arrives. Clearly, when the first task arrives ($\numtasks=1$), then
%$\nonhiredworkers^\numtasks=\workerset$ and
%$\hiredworkers^\numtasks=\emptyset$.
%For $\numtasks>1$, the values of $\hiredworkers^\numtasks$ and
%$\nonhiredworkers^\numtasks$ are updated in the last step (step 11) of
%the previous round and then we remove workers whose hiring interval
%finished in the previous step:
%
%\hspace{.4cm}$\mathcal{F}'\leftarrow\{r\in\workerset\St x(r,I_r^{\numtasks-\hireintervals_r}) = 1\}$
%
%\hspace{.4cm}$\hiredworkers^{\numtasks}\leftarrow\hiredworkers^{\numtasks}\setminus\mathcal{F}',\quad\nonhiredworkers^{\numtasks}\leftarrow\workerset\setminus\hiredworkers^{\numtasks}$
%
%\hspace{.4cm}\textbf{for each} $\worker{r}\in\mathcal{F}'$: \hspace{.4cm}set $\tilde{x}_r\leftarrow0$
%
%
%%\note[Aris]{Do we need fixed intervals?
%%Let the maximum length of an interval be $\hireintervals= {\tt max}_{r\in \workerset} \hireintervals_r$. 
%%}
%
%\item Let $\task{\numtasks}_\hiredworkers=\task{\numtasks}\cap\cup_{\worker{r}\in\hiredworkers^\numtasks}\worker{r}$
%be the skills from
%$\task{\numtasks}$ that are covered by already-hired workers and
%$\task{\numtasks}_\nonhiredworkers = \task{\numtasks}\setminus
%\task{\numtasks}_\hiredworkers$.
%
%\item For every skill $\askill\in\task{\numtasks}_\nonhiredworkers$ let
%$\poolUnhired{\askill}=\pool{\askill}\cap\nonhiredworkers^\numtasks$
%be the set of workers in $\nonhiredworkers^\numtasks$ such
%that every worker in $\poolUnhired{\askill}$ has skill $\askill$.
%Also let 
%\[\poolUnhiredUseful{\numtasks}=\cup_{\askill\in\task{\numtasks}_\nonhiredworkers}\poolUnhired{\askill}\]
%be the set of unhired workers that possess at least one skill required.
%
%\item \textbf{for each}
%$\worker{r}\in\poolUnhired{\askill}$:\hspace{.4cm}$\tilde{x}'_r\leftarrow \tilde{x}_r$
%
%\item \textbf{for each} skill $\askill\in\task{\numtasks}_\nonhiredworkers$:
%
%\hspace{.4cm} \textbf{while} $\sum_{r\in \pool{\askill}}\left(\tilde{x}_r+\tilde{f}_{r\numtasks}\right)<1$:
%
%\hspace{.8cm}$u_{\askill t}\leftarrow u_{\askill t}+1$
%
%\hspace{.8cm}\textbf{for each} $r\in \pool{\askill}$:\hspace{0.4cm}$\tilde{x}_r\leftarrow \tilde{x}_r\left(1+\frac{1}{\hiringcostwithsalary{r}}\right)+\frac{1}{\numworkers\hiringcostwithsalary{r}}$
%
%\hspace{.8cm}\textbf{for each} $r\in \pool{\askill}$:\hspace{0.4cm}$\tilde{f}_{r\numtasks}\leftarrow \tilde{f}_{r\numtasks}\left(1+\frac{1}{\outsourcecost{r}}\right)+\frac{1}{\numworkers\outsourcecost{r}}$
%
%\item \texttt{for each}
%$\worker{r}\in\poolUnhired{\askill}$:\hspace{.4cm}$\Delta \tilde{x}_r\leftarrow \tilde{x}_r-\tilde{x}'_r$
%
%
%\item $\hiredworkers'\leftarrow \emptyset$. 
%
%\item \textbf{repeat} $\rho_2$ times:
%    
%      \hspace{0.4cm}\textbf{for each}
%$r\in\poolUnhiredUseful{\numtasks}$
%    
%        \hspace{0.8cm}with probability $\Delta \tilde{x}_r$:
%    
%          \hspace{1.2cm}hire worker $\worker{r}$ (set
%    	  $x(r, I_r^\numtasks)\leftarrow1$, $\hiredworkers'\leftarrow\hiredworkers'\cup\{r\}$)%; \textbf{goto} 6
%
%        \hspace{0.8cm}with probability $\tilde{f}_{r\numtasks}$:
%
%          \hspace{1.2cm}outsource worker $\worker{r}$ (set $f_{r\numtasks}\leftarrow1$)%; \textbf{goto} 6
%
%
%\item \textbf{for each} skill $\askill\in\task{\numtasks}_\nonhiredworkers$:
%
%    \hspace{.4cm}\textbf{if} skill $\askill$ is not covered:
%
%    \hspace{.8cm}hire worker $\worker{r}$, $r\in\poolUnhired{\askill}$, with minimum cost $\hiringcost{r}$
%
%    \hspace{.8cm}(set $x(r, I_r^\numtasks)\leftarrow1$, $\hiredworkers'\leftarrow\hiredworkers'\cup\{r\}$)%; \textbf{goto} 6
%   
%\item $\hiredworkers^{\numtasks+1}=\hiredworkers^{\numtasks}\cup\hiredworkers'$.
%\end{enumerate}
%
%
%
%%\begin{enumerate}
%%
%%\item Let $\nonhiredworkers^\numtasks$ and $\hiredworkers^\numtasks$ represent the
%%workers that are not hired and hired, respectively, at the time that
%%$\task{\numtasks}$ arrives. Clearly, when the first task arrives ($\numtasks=1$), then
%%$\nonhiredworkers^\numtasks=\workerset$ and
%%$\hiredworkers^\numtasks=\emptyset$. For $\numtasks>1$ we set
%%$\hiredworkers^\numtasks\leftarrow\hiredworkers^{\numtasks-1} \setminus \{r: x(r,I_r^{\numtasks-\hireintervals_r})=1\}$.
%%Let the maximum length of an interval be $\hireintervals= {\tt max}_{r\in \workerset} \hireintervals_r$. 
%%%and $x_r=0$ for every $\worker{r}\in\workerset$.
%%
%%\item 
%%Also, let $\task{\numtasks}_\hiredworkers$ be the skills from $\task{\numtasks}$
%%that are covered by already-hired workers and $\task{\numtasks}_\nonhiredworkers = \task{\numtasks}\setminus \task{\numtasks}_\hiredworkers$.
%%  
%%
%%\item For every skill $\askill\in\task{\numtasks}_\nonhiredworkers$ let $P_\askill$ be the set of
%%  workers in $\nonhiredworkers^\numtasks$ such that every worker in
%%  $P_\askill$ has skill $\askill$.  
%%
%%\item For every skill $\askill\in\task{\numtasks}_\nonhiredworkers$ such that 
%%$$\sum_{r\in P_\ell}\left(f_{rt} + \sum_{I\in \intervals: t\in I} x(r,I) \right)<1$$ proceed as follows:
%%
%%  \begin{itemize}
%%  \item While $\sum_{r\in P_\ell}\left(f_{rt} + \sum_{I\in \intervals: t\in I} x(r,I) \right)<1$
%%    \begin{itemize}
%%    \item $u_{\askill t}=u_{\askill t}+1$
%%    \item For every $r\in P_\askill, I\in \intervals$: $x(r,I)=x(r,I) \left(1+\frac{1}{\hiringcostwithsalary{r}}\right)+\frac{1}{\numworkers\hiringcostwithsalary{r} \hireintervals_r}$
%%       \item For every $r\in P_\askill$: $f_{rt}=f_{rt}\left(1+\frac{1}{\outsourcecost{r}}\right)+\frac{1}{\numworkers\outsourcecost{r}}$
%%      \end{itemize}
%%   \end{itemize}
%%   \item Set $\hiredworkers' = \emptyset$. 
%%\item While there are skills in $\task{\numtasks}$ that remain uncovered repeat the following:
%%\begin{itemize}
%%\item For every worker $r\in P_\askill$
%%		\begin{itemize} 
%%			\item with probability $f_{rt}$ outsource worker $r$ (set $f_{rt}=1$).
%%			\item with probability $x(r,I)$ hire worker $r$ in interval $I$ (set $x(r,I)=1$, and $\hiredworkers'=\hiredworkers'\cup\{r\}$); 
%%		\end{itemize}
%%\end{itemize}
%%\item $\hiredworkers^{\numtasks+1}=\hiredworkers^{\numtasks}\cup\hiredworkers'$.
%%\end{enumerate}
%
%We call the above algorithm \altalgo.


%\subsection{Missing Proofs of Section~\protect\salarynewSectionNumber}
\subsection{Missing Proofs of Section~\ref{sec:salarynew}}

In this section we provide proofs for the theoretical results that
appear in Section~\ref{sec:salarynew}. We start with Theorem~\ref{thm:salary}:

\begin{theorem}[Theorem~\ref{thm:salary}]
\altalgo is an $O(\log\numworkers(\log
      \numskills+\log\maxoutsourcecost{r}+\log\numtasksTotal))$-competitive algorithm
 for  the \problemalternative problem.
\end{theorem}

\begin{proof}

The proof is very similar to that of Theorem~\ref{theorem:useforfree},
and it consists of the same three steps.
We assume that the algorithm has just processed
task~$\task{T}$.
(1)~First, we show the feasibility of the primal solution after the
arrival of $\task{\numtasks}$ and the assignment of values to the variables according to
\algouseforfree. (2)~Then, we show that after the completion of
$\task{\numtasks}$, the expected value of the obective function of the primal
LP (which we denote by $\PrimalTime{T}$) is, (essentially) at most
$3(\ln\numskills+\ln\maxoutsourcecost{r}+2\ln\numtasks)$ times the expected value of the
objective function of the dual LP (denoted by $\DualTime{T}$). In
particular, we show that
\[\begin{split}
\E{\PrimalTime{T}}
&\le 3(\ln\numskills+\ln\maxoutsourcecost{r}+2\ln\numtasks)\E{\DualTime{T}} + 2\\
&\le3(\ln\numskills+\ln\maxoutsourcecost{r}+2\ln\numtasks+1)\E{\DualTime{T}}.
\end{split}\]
This expectation is taken over the random choices of the algorithm when
rounding the fractional solution.
(3)~Finally, we  show that the dual solution is almost feasible, in
particular, we show that each dual constraint is violated by a factor of
at most $2\log\numworkers$.

As in Theorem~\ref{theorem:useforfree}, these three claims imply that
the solution produced by \altalgo is at most
\[3(\ln\numskills+\ln\maxoutsourcecost{r}+2\ln\numtasks+1)\cdot2\log\numworkers\]
worse than the optimal solution of the \problemalternative problem.
In the next paragraphs we perform these three steps.
To avoid repetition,
we present only the points where there is a difference from the
arguments in Theorem~\ref{theorem:useforfree}.

\spara{Analysis of feasibility of the primal LP:}
The proof is the same as in
Theorem~\ref{theorem:useforfree}: Step~9
guarantees that all the constraints in family
\eqref{eq:cover-skills-alt} are always satisfied.

\spara{Analysis of the primal and dual cost:}
The proof is identical to that of Theorem~\ref{theorem:useforfree}.
We note
that our algorithm guarantees that the dual objective is increased
(by~1) in step~5, only if a skill is not covered. Furthermore, the primal
increases when a worker $\worker{r}$ is being hired (lines 8 and~9), in
which case, for worker $\worker{r}$ only one variable
$x(r, I_r^{\numtasks})$ is set to~1, increasing the primal cost by
$\hiringcostwithsalary{r}$. Therefore, the analysis of the contribution
of step~8 to the primal remains intact, with the only syntactic change
that here we have variable
$x(r, I_r^{\numtasks})$
instead of variable $\tilde{x}_r$, $\hiringcostwithsalary{r}$
instead of~$\hiringcost{r}$, and $\rho_2(\numtasks)$ instead of $\rho_1$.

The analysis of the contribution of step~9 should be slightly modified
because, differently from
Theorem~\ref{theorem:useforfree}, a worker may
be outsourced multiple times. Therefore we need to bound the expected cost of
all these oursources that take place during the execution of step~9.
%(at most $\numtasksTotal$).
Arguing exactly as in Theorem~\ref{theorem:useforfree},
the probability that
the \textbf{if} statement of step~9 evaluates to true for a
skill~\askill is bounded by
%\[\frac1{\numskills\maxoutsourcecost{r}\numtasksTotal}.\]
\[\frac1{\numskills\maxoutsourcecost{r}\numtasks^2}.\]

%Following the line of reasoning of Theorem~\ref{theorem:useforfree},
%but applying a union bound not only over all skills (as we performed there)
%but also over all tasks that arrive, we obtain that the total expected
%increases to the objective function induced by operation performed by
%step~9 is bounded by~1.
(Of course, the analogous formula holds for $t\le\numtasks$.)
The proof then continues as the proof of
Theorem~\ref{theorem:useforfree}, just by substituting the bounding of
the total cost of step~9 up to the current task $\task{\numtasks}$,
given by inequality~\eqref{eq:Primal9}, with
\begin{equation*}
\E{\DeltaPrimalStep{\PrimalTimeStep{T}{9}}}
\le\sum_{t=1}^\numtasks \Card{\task{\numtasks}_\nonhiredworkers}\maxoutsourcecost{r}\cdot
\frac1{\numskills\maxoutsourcecost{r}t^2}
\le\sum_{t=1}^\numtasks\frac1{t^2}
\le\sum_{t=1}^\infty\frac1{t^2}
=\frac{\pi^2}6
<2.
%\le\frac1{\numskills\maxhiringcost{r}}\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\min_{r\in\poolUnhired{\askill}}\hiringcost{r}\le1,
\end{equation*}
Using this, we continue as in Theorem~\ref{theorem:useforfree} and we
obtain that
\[\E{\PrimalTime{T}}=\E{\PrimalTimeStep{T}{8}}+\E{\PrimalTimeStep{T}{9}}\le3\rho_2(\numtasks)\cdot\E{\DualTime{T}}+2.\]

\spara{Analysis of feasibility of the dual LP:} 
Again, the proof is similar to that of 
Theorem~\ref{theorem:useforfree}. Consider the family of
constraints~\eqref{eq:salary-alt-evict}. With the exact same argument as
in
Theorem~\ref{theorem:useforfree}, we have that, given a worker $\worker{r}$:
\begin{enumerate}
\item Any variable $u_{\askill t}$ with
$\askill\in\worker{r}$ may increase only if worker $\worker{r}$ is
not hired.
\item 
Given an interval $I\in\intervals$, if the total number of increments of variables $u_{\askill t}$
with $t\in I$ and $\askill\in\worker{r}$ is at least
$2\hiringcostwithsalary{r}\log\numworkers$, then variable
$\tilde{x}_r$ becomes at least~1.
\end{enumerate}
Consider now worker~$\worker{r}$ and a time interval $I\in\intervals$.
Assume that we have that
\[\sum_{t\in I} \sum_{\ell\in\task{t}\cap\worker{r}} u_{lt}
\ge2\hiringcostwithsalary{r} \log\numworkers.\]
Then, for the left-hand-side to increase, we need the arrival of a
task~$\task{t'}$ with $t'\le\numtasks$, such that (1) $t'\in I$ and (2) at least one skill
in $\task{t'}$ is possessed by worker $\worker{r}$. Consider any such skill
$\askill\in\task{t'}\cap\worker{r}$. Then, there are two cases that may
take place during the processing of task $\task{t'}$:
\begin{enumerate}
\item Worker $\worker{r}$ is hired. Then we have that 
$\askill\not\in\task{t'}_\nonhiredworkers$ so we do not enter
into step~5 and $u_{\askill t'}$ is not increased.
\item Worker $\worker{r}$ is not hired. Then, by the arguments we just
made, we have that $\tilde{x}_r\ge1$ and, therefore, 
\[\sum_{r\in \pool{\askill}}\left(\tilde{x}_r+\tilde{f}_{r\numtasks}\right)\ge1.\]
Consequently, neither in this case do we enter into step~5, so 
$u_{\askill t'}$ is not increased.
\end{enumerate}

Therefore, the family of constraints~\eqref{eq:salary-alt-evict} are
violated by a factor of at most $2\hiringcost{r}\log\numworkers$.

For the family of constraints~\eqref{eq:salary-alt-outsource} the proof
is identical to that of Theorem~\ref{theorem:useforfree}.
\end{proof}

Next we restate and prove Lemma~\ref{lemma:altTFOToTFO}.
The result is intuitive, although one has to take care of the
technicalities to prove it formally.


\begin{lemma}[Lemma~\ref{lemma:altTFOToTFO}]
The solution \SolTFOApprox to the \problemsalary problem
produced by the \algowithsalary algorithm is feasible for the
\problemsalary LP and has cost not higher than the cost of the 
\SolAltApprox solution to the \problemalternative problem that is
produced by the \altalgo algorithm.
\end{lemma}

\begin{proof}
First we prove the feasility of \SolTFOApprox. In particular, we need to
show that the families of constraints \eqref{eq:cover-skills-original} and
\eqref{eq:salary-constraint} are satisfied.

The feasibility of the
family \eqref{eq:cover-skills-original} follows directly from the
satisfiability of the family of constraints~\eqref{eq:cover-skills-alt}:
Recall that in both \SolTFOApprox and \SolAltApprox, the set of
variables $x(r,I)$ and $f_{rt}$ have the exact same values and the
constraints
\eqref{eq:cover-skills-original} and 
\eqref{eq:cover-skills-alt} are exactly the same.

Therefore it remains to prove the feasibility of the family constraints
\eqref{eq:salary-constraint}. Recall how we set the values of the
variables $g_{rt}$ in \SolTFOApprox: For each worker $\worker{r}$ and
each time step $t$, we set $x(r,I)=1$ if there exists an
$I\in\intervals$ such that $t\in I$, and 0 otherwise. Therefore, to
make sure that no constraint \eqref{eq:salary-constraint} is violated,
we should prove that there does not exist a time step $t$ and two
intervals $I,I'$ with $I\ne I'$ and $t\in I,I'$ such that
$x(r,I)=x(r,I')=1$. Intuitively, this cannot not happen: it would mean that
we decided to hire worker \worker{r} even if he is already
hired. Let us see now formally why this cannot happen. Assume that this
is not the case, and assume that for intervals $I,I'$ we have
$x(r,I)=x(r,I')=1$ even though $I\cap I'\ne\emptyset$.
Let $I=[t_I, \dots, t_I+\hireintervals_r-1]$ and 
$I'=[t_{I'}, \dots, t_{I'}+\hireintervals_r-1]$, and assume without loss of
generality that $t_I<t_{I'}$.
The fact that $I\cap I\ne\emptyset$ implies that $t_I\in I$.

We claim that for each $t\in I$ we have that
$\worker{r}\cap\task{t}_\nonhiredworkers=\emptyset$. At time
step $t_I$, during step 8, we set $x(r,I)=1$ and during step 10 we add
$r$ into $\hiredworkers^{t_I+1}$. Note that $r$ remains into the set
$\hiredworkers^{t}$ for $t\le t_I+\hireintervals_r-1$ (steps 1 and~10).
Therefore, for each $t\in[t_I+1, t_I+\hireintervals_r-1]$ (i.e., for
each $t\in I$) we have that
\[\task{t}_\nonhiredworkers=\task{t}\setminus\task{t}_\hiredworkers
= \task{t}\setminus\cup_{r'\in\hiredworkers^t}\worker{r'},\]
and, because $r\in\hiredworkers^t$, we have that
$\worker{r}\cap\task{t}_\nonhiredworkers=\emptyset$.

This fact applied to time step $t_{I'}\in I$ gives that
$\worker{r}\cap\task{t_{I'}}_\nonhiredworkers=\emptyset$.
In other words, for each $\askill\in\task{t_{I'}}_\nonhiredworkers$, we have
that $\askill\not\in\pool{\askill}$ (recall that $\pool{\askill}$ is the
set of workers who possess skil $\askill$). Therefore, $\tilde{x}_r$ will not
increase during step~5 in the processing of task~$t_{I'}$, which implies
(step~6) that $\Delta\tilde{x}_r=0$, and in turn means that, during
step~8, worker $\worker{r}$ cannot be hired and, thus, we cannot have
$x(r,I')=1$,
leading to a contradiction.

As a consequence, for each $t$ we have that there exists at most one
interval $I\in\intervals$ with $t\in I$ such that $x(r,I)=1$.
Therefore, the family of constraints \eqref{eq:salary-constraint} is
satisfied, and $\SolTFOApprox$ is a feasible solution for the
\problemsalary LP.

We now turn our attention to the cost. First notice that
\[\begin{split}
\sum_{t=1}^{\numtasks} \salary{r}  g_{rt}
&\stackrel{{\mathclap{\textrm{(a)}}}}{\le}\sum_{t\in\cup_{I\in\intervals}I}\salary{r}  g_{rt}
%&=\sum_{t\in\{t'\in\{1, \dots, \numtasks\}\St g_{rt'}=1\}}\salary{r}\\
\stackrel{{\mathclap{\textrm{(b)}}}}{=}\sum_{\substack{t\in\cup_{I\in\intervals}I\\
  g_{rt}=1}}\salary{r}
\stackrel{{\mathclap{\textrm{(c)}}}}{=}\sum_{\substack{t\in\cup_{I\in\intervals}I\\
  t:\ \exists I \text{ s.t. } t\in I \text{ and } x(r,I)=1}}\salary{r}\\
&\stackrel{{\mathclap{\textrm{(d)}}}}{=}\sum_{I\in\intervals}\ \sum_{t\in I:\ x(r,I)=1}\salary{r}
\stackrel{{\mathclap{\textrm{(e)}}}}{=}\sum_{\substack{I\in\intervals\\
I:\ x(r,I)=1}}
\salary{r}\hireintervals_r
=\sum_{I\in\intervals}\salary{r}\hireintervals_rx(r,I)\\
&\le\sum_{I\in\intervals}\salary{r}\left(\frac{\hiringcost{r}}{\salary{r}}+1\right)\hireintervals_rx(r,I)
\stackrel{{\mathclap{\textrm{(f)}}}}{\le}\sum_{I\in\intervals}2\hiringcost{r}x(r,I),
\end{split}\]
where $\textrm{(a)}$ is true because $\cup_{I\in\intervals}I$
are all the positive integers,
$\textrm{(b)}$ because \algowithsalary sets $g_{rt}=0$ or $g_{rt}=1$,
$\textrm{(c)}$ because \algowithsalary sets $g_{rt}=1$ if and only if
there exists some interval $I\in\intervals$ such that $t\in I$ with
$x(r,I)=1$,
$\textrm{(d)}$ because, as we showed, for each $t$ there can at most one
$I\in\intervals$ with $t\in I$ with $x(r,I)=1$, 
$\textrm{(e)}$ because, \altalgo sets $x(r,I)=1$ only for intervals $I$
with $\Card{I}=\hireintervals_r$ (step~8), and
$\textrm{(f)}$ because we have
$\salary{r}\le\hiringcost{r}$.
The result follows by comparing the objective functions of the LP for
\problemsalary and \problemalternative, and using the inequality that we
proved, and the fact that $\hiringcostwithsalary{r}=3\hiringcost{r}$.
\end{proof}


Lemma~\ref{lemma:factor} will allow us to relate the cost of a solution
to \problemalternative to a solution to \problemsalary. We restate it
and we prove it:

%\begin{lemma}[Lemma~\ref{lemma:factor}]
%If $P^{\text{Alt}}$ is the cost of any feasible solution to the {\problemalternative}
%and $P^{\text{Tfo}}$ the cost of the same solution when transformed to a solution of
%{\problemsalary} using the last step of {\algowithsalary}, then we have that
%$P^{\text{Alt}}\leq 3 P^{\text{Tfo}}$.
%\end{lemma}

\begin{lemma}[Lemma~\ref{lemma:factor}]
Consider any solution $\SolutionTFO$ to \problemsalary with cost $\CostSolutionTFO$. This
solution can be converted to a solution $\SolutionAlt$ for \problemalternative with a
cost of at most $3\CostSolutionTFO$.
%
%If $P^{\text{Alt}}$ is the cost of any feasible solution to the {\problemalternative}
%and $P^{\text{Tfo}}$ the cost of the same solution when transformed to a solution of
%{\problemsalary} using the last step of {\algowithsalary}, then we have that
%$P^{\text{Alt}}\leq 3 P^{\text{Tfo}}$.
\end{lemma}

\begin{proof}
We construct the feasible solution $\SolutionAlt$ for the LP corresponding to {\problemalternative} 
whose cost is at most 3 times higher. We look at the variables of the
solution for the LP of \problemsalary given by \SolutionTFO, and we
describe how we set the variables for the LP corresponding to \problemalternative.

We argue separately for each individual worker~$\worker{r}$.
We consider a period $\Pi$ consisting of two consecutive time periods, $I_F$, during which $\worker{r}$
is not hired in $\SolutionTFO$, and $I_H$, during which $\worker{r}$ is hired.  Let $O\subseteq I_F$ 
be the set of times when $\worker{r}$ is outsourced.  

The contribution of worker $\worker{r}$ to the cost of $\SolutionTFO$
during $\Pi$ is
\[\CostPeriodTFO\Def\outsourcecost{r}\cdot\Card{O}+\hiringcost{r}+\salary{r}\cdot\Card{I_H}.\]

For each $t\in I_F$ we set $x(r,[t,t+\hireintervals_r-1])=0$. For each $t\in O$ we
set $f_{rt}=1$, otherwise $f_{rt}=0$. That is, we choose to outsource
in $\SolutionAlt$ when
$\SolutionTFO$ outsources. Finally, we keep hired $\worker{r}$ during the entire
period $I_H$ by hiring at the beginning of $I_H$, firing after $\hireintervals_r$
steps, directly rehiring, and so on. Formally, let $I_H=[t_1, t_{\ell}]$. Let
$t_2=t_1+\hireintervals_r$, $t_3=t_2+\hireintervals_r$, and so on until we arrive at some $i^*$
such that $t_{\ell}\in[t_{i^*}, t_{i^*}+\hireintervals_r-1]$.
For each $i=1,\dots,i^*$ we set $x(r, [t_i, t_i+\hireintervals_r-1])=1$,
and we set all the other $x(r,[t,t+\hireintervals_r-1])=0$ (for $t\in I_H$).

We first bound the cost of worker $\worker{r}$ during $\Pi$, which will
lead to a bound on the cost of the entire $\SolutionAlt$. At the end we also prove
the feasibility of $\SolutionAlt$. The cost $\CostPeriodAlt$ of worker $\worker{r}$ in
$\SolutionAlt$ during period $\Pi$ is equal to
\[\CostPeriodAlt=i^*\cdot\hiringcostwithsalary{r}+\Card{O}\cdot\outsourcecost{r}.\]
We have that
\[i^*=\Ceil{\frac{\Card{I_H}}{\hireintervals_r}}\le\frac{\Card{I_H}}{\Ceil{\hiringcost{r}/\salary{r}}}+1\le
\frac{\Card{I_H}}{\hiringcost{r}/\salary{r}}+1
=\frac{\Card{I_H}\cdot\salary{r}+\hiringcost{r}}{\hiringcost{r}},\]
and 
$\hiringcostwithsalary{r}=3\hiringcost{r}$,
so the cost is
\[\begin{split}
\CostPeriodAlt&=\frac{\Card{I_H}\cdot\salary{r}+\hiringcost{r}}{\hiringcost{r}}\cdot3\hiringcost{r}+\Card{O}\cdot\outsourcecost{r}\\
&=3(\Card{I_H}\cdot\salary{r}+\hiringcost{r})+\Card{O}\cdot\outsourcecost{r}.\\
\end{split}\]

The ratio is
\[\frac{\CostPeriodAlt}{\CostPeriodTFO}=
\frac{3\cdot\Card{I_H}\cdot\salary{r}+3\cdot\hiringcost{r}+\Card{O}\cdot\outsourcecost{r}}
{\salary{r}\cdot\Card{I_H}+\hiringcost{r}+\outsourcecost{r}\cdot\Card{O}}\le3,\]
by applying Lemma~\ref{lem:ratio_sums}.

This holds for a given worker and a given period $\Pi$. To compute the total cost
of $\SolutionTFO$ we should sum over all worker and over all the periods
$\Pi$ the cost of worker $\worker{r}$ during~$\Pi$. Similarly, for $\SolutionAlt$. For each of those the
ratio is bounded by 3, therefore, by applying once more
Lemma~\ref{lem:ratio_sums}, we can conclude that the cost of
$\SolutionAlt$ is at most 3 times the cost of
$\SolutionTFO$.\footnote{Note that for a given worker $\worker{r}$, in
the last period we may not hire in \SolutionTFO. Then we do not hire in
\SolutionAlt either and we have that $\Card{I_H}=\emptyset$, and
$\CostPeriodTFO=\CostPeriodAlt=\outsourcecost{r}\cdot\Card{O}$, so the
ratio of~3 between the two costs still holds.}


Finally, we show that our solution is feasible, that is that constraint
\eqref{eq:cover-skills-alt} is satisfied. To prove that, first notice that by our
construction, if a worker $\worker{r}$ is outsourced in $\SolutionTFO$,
then he is also outsourced in $\SolutionAlt$.
Formally, for each $t\in O$, in \SolutionAlt we set $f_{rt}=1$.
Similarly, if $\worker{r}$
is hired in $\SolutionTFO$ then he is also hired in
$\SolutionAlt$. Formally,
for every $t\in I_H$ there exists an interval
$[t_i, t_i+\hireintervals_r-1]$ such that $t\in [t_i, t_i+\hireintervals_r-1]$ with
$x(r,[t_i, t_i+\hireintervals_r-1])=1$ in \SolutionAlt. Informally, in
\SolutionAlt during
interval $I_H$, worker $\worker{r}$ is always hired because, as soon as
he is fired, we rehire him.
This fact, along with the fact that
constraint~\eqref{eq:cover-skills-original} is satisfied (as
    \SolutionTFO is a feasible solution), implies that
constraint~\eqref{eq:cover-skills-alt} is satisfied.\footnote{It
may happen in our construction for $\SolutionAlt$ that we decide to both hire and outsource
a worker $\worker{r}$ at some time point $t$. Formally, it may happen
that we have $x(r,[t',t'+\hireintervals_r-1])=1$ for some $t\in
[t',t'+\hireintervals_r-1]$ and also $f_{rt}=1$. This may happen because
in $\SolutionAlt$ we hire for intervals of length $\hireintervals_r$,
thus, we may have worker $\worker{r}$ hired when the interval $I_H$ of
the next period $\Pi$ starts. Nevertheless, this does not
invalidate constraint~\eqref{eq:cover-skills-alt}. A better solution
will set $f_{rt}=0$ in such a case.}
%follows from constraint
%\eqref{eq:cover-skills-original}. It guarantees that for each required
%skill a worker either is hired ($g_{rt}=1$, which takes place for $t\in I_H$)
%or outsourced ($f_{rt}=1$, which takes place for $t\in I_F$). For the
%first case, note that for every $t\in I_H$ there exists an interval
%$[t_i, t_i+\hireintervals_r-1]$ such that $t\in [t_i, t_i+\hireintervals_r-1]$ with
%$x(r,[t_i, t_i+\hireintervals_r-1])=1$. Informally, in the alternate formulation, during
%interval $I_H$ worker $\worker{r}$ is always hired because as soon as he is fired
%we rehire him. For the latter case, for each $t\in O$ we have set
%$f_{rt}=1$. Therefore, constraint~\eqref{eq:cover-skills-alt} is satisfied.
\end{proof}



%The analysis below, provides a proof to the above proposition, is
%heavily based on Section~\ref{sec:useforfree}. It has one additional
%step to show the relationship between the solution of the alternative
%formulation and the original problem. More specifically:
%(1) First, we show the feasibility of the primal solution after the arrival of
%$\task{T}$ and the assignment of values to the variables according to
%\altalgo. (2) Then we show 
%$\E{\PrimalTime{T}}\le 3(\ln\numskills+\ln\maxhiringcost{r})\E{\DualTime{T}} + 1$.
%This is the same result with Section~\ref{sec:useforfree}, with the
%difference that here the value $\rho$ is higher.
%(3) Again, as in Section~\ref{sec:useforfree}, we show that each
%dual constraint is violated by a factor of $2\log\numworkers$.
%(4) The final step is new in this section. We prove that the solution obtained above for the \problemalternative problem can be transformed into a feasible
%solution to the original (\problemsalary) problem by keeping all common variables set as above and setting
%$g_{rt}=1$ for each $r, t\in I$ for which
%$x(r,I)=1$, and 0 otherwise. This induces an multiplicative additional
%factor of~3 to the approximation ratio. We refer to the algorithm that takes the output of \altalgo and performs this
%transformation as the \algowithsalary algorithm.
%
%Putting everything together, we obtain the result.
%
%In the next paragraphs we perform these four steps. To avoid repetition,
%we only present only the points where there is a difference from the
%arguments in Section~\ref{sec:useforfree}.

Theorem~\ref{thm:salaryfinal}, proven next, is the main theorem of
Section~\ref{sec:salarynew}.

\begin{theorem}[Theorem~\ref{thm:salaryfinal}]
\algowithsalary is an $O(\log\numworkers(\log
      \numskills+\log\maxoutsourcecost{r}+\log\numtasks))$-competitive algorithm
 for  the \problemsalary problem.
\end{theorem}

\begin{proof}
Consider the following solutions:
\begin{itemize}
\item \SolTFOOpt: The optimal solution of the \problemsalary problem.
\item \SolAltFromTFOOpt: The solution to \problemalternative that we
obtain if we apply the transformation of Lemma~\ref{lemma:factor} to
\SolTFOOpt.
\item \SolAltOpt: The optimal solution of the \problemalternative problem.
\item \SolTFOApprox: The solution to \problemsalary given by algorithm \algowithsalary.
\item \SolAltApprox:The solution to \problemalternative given by algorithm \altalgo.
\end{itemize}
Let $\gamma$ be the approximation ratio of algorithm \altalgo,
guaranteed by Theorem~\ref{thm:salary}. We have that
$\gamma=O(\log\numworkers(\log \numskills+\log\maxoutsourcecost{r}+\log\numtasks))$.

Given a solution $\SolutionLetter$ to the \problemsalary or
\problemalternative problems, we denote by
$\CostOfSolution{\SolutionLetter}$ its expected cost.

By Lemma~\ref{lemma:altTFOToTFO} we have that
$\CostOfSolution{\SolTFOApprox}\le\CostOfSolution{\SolAltApprox}$.
By Theorem~\ref{thm:salary} we have that
$\CostOfSolution{\SolAltApprox}\le\gamma\cdot\CostOfSolution{\SolAltOpt}$.
From the optimality of \SolAltOpt, we have that
$\CostOfSolution{\SolAltOpt}\le\CostOfSolution{\SolAltFromTFOOpt}$.
Finally, from Lemma~\ref{lemma:factor}, that
$\CostOfSolution{\SolAltFromTFOOpt}\le 3\CostOfSolution{\SolTFOOpt}$.
Putting everything together, we obtain that
\[\CostOfSolution{\SolTFOApprox}\le\CostOfSolution{\SolAltApprox}
\le\gamma\cdot\CostOfSolution{\SolAltOpt}\le\gamma\cdot\CostOfSolution{\SolAltFromTFOOpt}\le
3\gamma\cdot\CostOfSolution{\SolTFOOpt}.
\]
\end{proof}


==> simple-proofs.tex <==
We restate Theorem~\ref{theorem:useforfree}:

\begin{theorem}[Theorem~\ref{theorem:useforfree}]
%  \sloppy
  \algouseforfree is an
$O(\log\numworkers(\log\numskills+\log\maxhiringcost{r}))$- competitive algorithm
 for  the \problemuseforfree problem, where
 $\maxhiringcost{r}=\max_{\worker{r}\in\workerset}\hiringcost{r}$.
\end{theorem}


\begin{proof}

The structure of the proof is the one followed by Buchbinder and
Naor~\cite{buchbinder2009design}, when they presented the online
primal--dual approach and it consists of
three steps. We assume that the algorithm has just processed
task~$\task{T}$.
(1)~First, we show the feasibility of the primal solution after the
arrival of $\task{\numtasks}$ and the assignment of values to the variables according to
\algouseforfree. (2)~Then, we  show that after the completion of
$\task{\numtasks}$, the expected value of the obective function of the primal
LP (which we denote by $\PrimalTime{T}$) is, (essentially) at most
$3(\ln \numskills+\ln\maxhiringcost{r})$ times the expected value of the
objective function of the dual LP (denoted by $\DualTime{T}$). In
particular, we show that
\[\E{\PrimalTime{T}}\le
3(\ln\numskills+\ln\maxhiringcost{r})\E{\DualTime{T}} + 1
\le3(\ln\numskills+\ln\maxhiringcost{r}+1)\E{\DualTime{T}}.\]
This expectation is taken over the random choices of the algorithm when
rounding the fractional solution.
(3)~Finally, we  show that the dual solution is almost feasible, in
particular, we show that each dual constraint is violated by a factor of
at most $2\log\numworkers$.
%
%
%(1) First, we show the feasibility of the primal solution after the
%arrival of $\task{\numtasks}$ and the assignment of values to the variables according to
%\algouseforfree. (2) Then, we essentially show that after the completion of
%$\task{\numtasks}$, the expected value of the obective function of the primal
%LP (which we denote by $\PrimalTime{T}$) is at most 
%$3(\ln \numskills+\ln\maxhiringcost{r})$ times the expected value of the
%objective function of the dual LP (denoted by $\DualTime{T}$). In particular we
%show that $\E{\PrimalTime{T}}\le
%3(\ln\numskills+\ln\maxhiringcost{r})\E{\DualTime{T}} + 1$.
%This expectation is taken over the random choices of the algorithm when
%rounding the fractional solution.
%(3) Finally, we  show that the dual solution is almost feasible, in
%particular, we show that each dual constraint is violated by a factor of
%at most $2\log\numworkers$.
  
Then, as shown in~\cite{buchbinder2009design}, it follows that the
algorithm maintains a feasible solution at an expected cost that is at
most a factor
\[3(\ln\numskills+\ln\maxhiringcost{r}+1)\cdot 2\log\numworkers\]
higher than the optimal offline solution.

In the next paragraphs we perform these three steps.

\spara{Analysis of feasibility of the primal LP:}
The primal program has only a set of
constraints~\eqref{eq:tfo-lump-sum-primal} (except for the nonnegativity
constraints, which remain trivially satisfied), and here we prove their feasibility.

First consider constraints involving the
current time instance $\numtasks$. The skills in
$\task{\numtasks}_\hiredworkers=\task{\numtasks}\setminus
\task{\numtasks}_\nonhiredworkers$ are (by the definition of
$\task{\numtasks}_\hiredworkers$) the skills covered by already
hired workers, that is, for each 
$\askill\in\task{\numtasks}_\hiredworkers$ there exists a worker
$\worker{r}$ with $r\in \pool{\askill}$ such that $x_r=1$. For 
$\askill\in\task{\numtasks}_\nonhiredworkers$, during the execution of
step~8 a worker $\worker{r}$ who possesses the skill may either
be hire (setting $x_r=1$) or outsourced (setting $f_{r\numtasks}=1$). In the
case that none of these happens, step~9
guarantees that every required skill that has not been covered up to that point
(either by hiring a worker or by outsourcing) eventually becomes
covered by hiring a worker $\worker{r}$ possessing the skill,
ensuring that we always have for an $r\in \pool{\askill}$, $x_r=1$ or
$f_{r\numtasks}=1$.
  
%Step~6 of our algorithm guarantees
%that with probability~1 the constraint will eventually be satisfied: We
%keep attempting to hire or to outsource some worker until one of the two
%happens and notice that in that case the constraint is satisfied.
%Furthermore, step~4 guarantees that, for each
%$\askill\in\task{\numtasks}_\nonhiredworkers$, at least one of $f_{rt}$ or
%an $x_r\in\pool{\askill}$ is strictly greater than~0.

For $t=1,\dots, \numtasks-1$, 
constraint~\eqref{eq:tfo-lump-sum-primal} is satisfied from the previous
tasks that have arrived, and from the fact that, as we mentioned
previously, the values of the variables do not decrease as time passes.


%for each uncovered skill $\askill$ we have
%By construction the
%algorithm ensures that skills are fractionally covered for all tasks, so the primal
%constraints \eqref{eq:tfo-lump-sum-primal} are always satisfied.

\spara{Analysis of primal and dual cost:}
We will now relate the cost of the primal and the dual solutions produce
by our algorithm 
after task \task{\numtasks} is processed and before potential task
\task{\numtasks+1} arrives.
%We now analyze the difference of the objective values of the primal
%and the dual LPs after task \task{\numtasks} and before potential task
%\task{\numtasks+1}. We
%denote the former by $\DeltaPrimalTime{T}$ and the latter by
%$\DeltaDualTime{T}$.
%Denote the former by $\PrimalTime{T}$ and the latter by $\DualTime{T}$.

Note that the primal may increase in lines 8 and 9. Let $\PrimalTimeStep{T}{8}$
and $\PrimalTimeStep{T}{9}$ be the cost induced by operations performed
in step 8 and step 9, respectively, such that
$\PrimalTime{T}=\PrimalTimeStep{T}{8}+\PrimalTimeStep{T}{9}$. We will
bound the expected contribution each of the two
component separately. In particular, we will prove that
\[\E{\PrimalTimeStep{T}{8}}\le3\rho_1\cdot\E{\DualTime{T}},\]
and that
\[\E{\PrimalTimeStep{T}{9}}\le1.\]

To prove the former, we start by counting the increase of the
variables that occurs in step~5, during the processing of task $\task{T}$.
%Call this cost $\DeltaPrimalTimeStep{T}{5}$.
%, and let us
%denote the corresponding increase causes during the execution of
%step~$i$ by
%$\DeltaPrimalTimeStep{T}{i}$, such that,
%$\DeltaPrimalTime{T}=\sum_{i\in\{8,9,10\}}\DeltaPrimalTimeStep{T}{i}$.
%The dual increases only during the execution of step~5. We will bound
%all these increases.
We need some additional definitions. Consider a worker $\worker{r}\in
\poolUnhiredUseful{\numtasks}$
(recall that these are the unhired workers who possess at least one
 uncovered skill of task $\numtasks$ and note that they are the
 workers whose values $\tilde{x}_r$, $x_r$,
 $\tilde{f}_{r\numtasks}$, or $f_{r\numtasks}$ may have been
updated during during the processing of task~$\numtasks$). This is a
worker who is not hired during the arrival of task~$\numtasks$.
The value $\tilde{x}_r$ corresponding to this worker may have increased because of
previous tasks or the current task.
%, and which in the current task $\numtasks$ it may have increased in
%steps 5, 8, and 9. For the previous tasks it may have increased only
%during step 5 (because $\worker{r}$ is not hired) and for the current
%task we consider, for now, only the increase during step~5.
Assume that it has increased during $\nu_r$ tasks (including the current
one) and let $\Delta \tilde{x}_r^i$ be the $i$th such increase, such that,
at the end of the execution of step~5 of the current task we have
\begin{equation}
\label{eq:xr}
\tilde{x}_r=\sum_{i=1}^{\nu_r}\Delta\tilde{x}_r^i.
\end{equation}

In particular, notice that the total increase during step~5 of the
current task is
$\Delta\tilde{x}_r^{\nu_r}$. For each skill $\askill$ we let $\Delta\tilde{x}_{r,\askill}$
to be the increase of $\tilde{x}_r$ during the consideration of skill
$\askill$ when processing task~\numtasks.
Then we have that
\begin{equation}
\label{eq:deltaxrnur}
\Delta
\tilde{x}_r^{\nu_r}=\sum_{\askill\in\task{\numtasks}_\nonhiredworkers\cap\worker{r}}
\Delta \tilde{x}_{r,\askill}.
\end{equation}

Analogously, define $\tilde{f}_{rT,\askill}$ be the increase of variable
$\tilde{f}_{rT}$, such that
\begin{equation}
\label{eq:frT}
\tilde{f}_{rT}=\sum_{\askill\in\task{\numtasks}_\nonhiredworkers\cap\worker{r}}
\tilde{f}_{rT,\askill}.
\end{equation}
(Note that, differently from $\tilde{x}_r$, $\tilde{f}_{rT}$ is 0 before the execution
of step~5.)


The increase $\Delta\tilde{x}_{r,\askill}$ has taken place during the execution
of the \textbf{while} loop of step~5, so let $\chi_{r,\askill}^i$ be 
the $i$th such increase of $\tilde{x}_r$, such that
\begin{equation}
\label{eq:deltaxrell}
\Delta\tilde{x}_{r,\askill}=\sum_{i=1}^{\kappa_{\askill}}\chi_{r,\askill}^i,
\end{equation}
where $\kappa_{\askill}$ is the number of times that the \textbf{while}
loop was executed for skill~$\askill$.


Similarly, let $\phi_{rT,\askill}^i$ be the corresponding increase of
$\tilde{f}_{rT,\askill}$, which gives
\begin{equation}
\label{eq:frTell}
\tilde{f}_{rT,\askill}=\sum_{i=1}^{\kappa_{\askill}}\phi_{rT,\askill}^i,
\end{equation}


Now we are ready to analyze the increase of the primal and the dual. The
latter is easy: each time that the \textbf{while} loop of step~5 is
executed, it increases by~1 (exactly one variable $u_{\askill T}$
increases by~1). Therefore, we have that
\begin{equation}
\label{eq:DeltaDual}
\DeltaDualTime{T}=\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_\askill.
\end{equation}

Now we move to the primal. Note that the only variables $f_{rt}$ that are
being updated are variables $f_{rT}$ and only workers in 
$\poolUnhiredUseful{\numtasks}$ may update their values $x_r$ and $f_{rT}$.
Therefore, we study the increase of those variables.

%For the increase $\DeltaPrimalTimeStep{T}{5}$ note that $x_r$ has
%changed by $\Delta\tilde{x}_r^{\nu_r}$ and only $f_{rT}$ may have changed.
%Therefore,
%\[\begin{split}
%\DeltaPrimalTimeStep{T}{5}
%&=\sum_{r\in\poolUnhiredUseful{\numtasks}}
%\left(\hiringcost{r}\cdot\Delta\tilde{x}_r^{\nu_r}+\outsourcecost{r}\cdot f_{rT}\right)\\
%&\stackrel{\mathclap{\eqref{eq:deltaxrnur},\eqref{eq:frT}}}{=}
%\ \sum_{r\in\poolUnhiredUseful{\numtasks}}
%\left(\hiringcost{r}\cdot\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
%\Delta\tilde{x}_{r,\askill}+\outsourcecost{r}\cdot
%\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
%f_{rT,\askill}\right)\\
%&\stackrel{\mathclap{\textrm{(a)}}}{=}\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
%\sum_{r\in\poolUnhired{\askill}}
%\left(\hiringcost{r}\cdot\Delta\tilde{x}_{r,\askill}+\outsourcecost{r}\cdot f_{rT,\askill}\right)\\
%&\stackrel{\mathclap{\eqref{eq:deltaxrell},\eqref{eq:frTell}}}{=}
%\ \sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
%\sum_{r\in\poolUnhired{\askill}}
%\left(\hiringcost{r}\cdot\sum_{i=1}^{\kappa_{\askill}}\chi_{r,\askill}^i
%+\outsourcecost{r}\cdot \sum_{i=1}^{\kappa_{\askill}}\phi_{rT,\askill}^i\right)\\
%&=\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
%\sum_{i=1}^{\kappa_{\askill}}\sum_{r\in\poolUnhired{\askill}}
%\left(\hiringcost{r}\cdot\chi_{r,\askill}^i +\outsourcecost{r}\cdot\phi_{rT,\askill}^i \right),
%\end{split}\]
%where $\textrm{(a)}$ follows from the fact that
%$\poolUnhiredUseful{\numtasks}=\cup_{\askill\in\task{\numtasks}_\nonhiredworkers}
%\poolUnhiredUseful{\askill}$.
%Let us now consider a particular increase
%$\chi_{r,\askill}^i$ of $x_r$ and
%$\phi_{rT,\askill}^i$ of $f_{rT}$. Assume that the corresponding values
%before the increase were
%$x_r^{\text{old}}$ and $f_{rT}^{\text{old}}$.
%
%Then we have that
%\[\begin{split}
%\chi_{r,\askill}^i
%&=x_r^{\text{old}}\left(1+\frac{1}{\hiringcost{r}}\right)+\frac{1}{\numworkers\hiringcost{r}}-
%x_r^{\text{old}}\\
%&=\frac{1}{\hiringcost{r}}\cdot\left(x_r^{\text{old}}+\frac1n\right)
%\end{split}\]
%and
%\[\phi_{rT,\askill}^i=\frac{1}{\outsourcecost{r}}\cdot\left(f_{rT}^{\text{old}}+\frac1n\right).\]
%
%Furthermore, because we entered the \textbf{while} loop, we have that
%\[\sum_{r\in\poolUnhired{\askill}}\left(x_r^{\text{old}}+f_{rT}^{\text{old}}\right)
%=\sum_{r\in\pool{\askill}}\left(x_r^{\text{old}}+f_{rT}^{\text{old}}\right)<1.\]
%(The equality is because only unhired worker possess skill~$\askill$.)
%
%Using all these facts we obtain that
%\begin{equation}
%\label{eq:DeltaPrimal5}
%\DeltaPrimalTimeStep{T}{5}
%<\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\sum_{i=1}^{\kappa_{\askill}}\left(1+\frac{2\Card{\poolUnhired{\askill}}}n\right)
%\le3\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill},
%\end{equation}
%using the fact that $\Card{\poolUnhired{\askill}}\le n$.

We start by calculating the \emph{expected} increase
$\DeltaPrimalTimeStep{T}{8}$ induced by the execution of step~8.
For each of $\rho_1$
trials we hire worker $\worker{r}$ with probability $\Delta\tilde{x}_r$ and in
this case the variable $x_r$ (and, therefore, the objective value of the
primal LP) will increase by~\hiringcost{r}. Similarly, we outsource a worker
$\worker{r}$ with probability~$\tilde{f}_{rT}$. Therefore, we can bound
\[\begin{split}
\E{\DeltaPrimalTimeStep{T}{8}}
&\le\rho_1\sum_{r\in\poolUnhiredUseful{\numtasks}}
\left(\hiringcost{r}\cdot\Delta\tilde{x}_r^{\nu_r}+\outsourcecost{r}\cdot \tilde{f}_{rT}\right),\\
&\stackrel{\mathclap{\eqref{eq:deltaxrnur},\eqref{eq:frT}}}{=}
\ \rho_1\sum_{r\in\poolUnhiredUseful{\numtasks}}
\left(\hiringcost{r}\cdot\sum_{\askill\in\task{\numtasks}_\nonhiredworkers\cap\worker{r}}
\Delta\tilde{x}_{r,\askill}+\outsourcecost{r}\cdot
\sum_{\askill\in\task{\numtasks}_\nonhiredworkers\cap\worker{r}} \tilde{f}_{rT,\askill}\right)\\
&\stackrel{\mathclap{\textrm{(a)}}}{=}
\rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
\sum_{r\in\poolUnhired{\askill}}
\left(\hiringcost{r}\cdot\Delta\tilde{x}_{r,\askill}+\outsourcecost{r}\cdot \tilde{f}_{rT,\askill}\right)\\
&\stackrel{\mathclap{\eqref{eq:deltaxrell},\eqref{eq:frTell}}}{=}
\ \rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
\sum_{r\in\poolUnhired{\askill}}
\left(\hiringcost{r}\cdot\sum_{i=1}^{\kappa_{\askill}}\chi_{r,\askill}^i
+\outsourcecost{r}\cdot \sum_{i=1}^{\kappa_{\askill}}\phi_{rT,\askill}^i\right)\\
&=\rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}
\sum_{i=1}^{\kappa_{\askill}}\sum_{r\in\poolUnhired{\askill}}
\left(\hiringcost{r}\cdot\chi_{r,\askill}^i +\outsourcecost{r}\cdot\phi_{rT,\askill}^i \right),
\end{split}\]
where $\textrm{(a)}$ follows from the fact that
$\poolUnhiredUseful{\numtasks}=\cup_{\askill\in\task{\numtasks}_\nonhiredworkers}
\poolUnhiredUseful{\askill}$ (in words, in both cases we sum the
variables
$\Delta\tilde{x}_{r,\askill}$
and
$\tilde{f}_{rT,\askill}$ of all uncovered skills $\askill$ of task
$\numtasks$ and of all (unhired) workers who possess skill \askill).
%For a formal proof, note that we have:
%\[\begin{split}
%\left\{(r,\askill)\St r\in\poolUnhiredUseful{\numtasks},\askill\in\task{\numtasks}_\nonhiredworkers\cap\worker{r}\right\}
%&=\left\{(r,\askill)\St r\in\bigcup_{\askill\in\task{\numtasks}_\nonhiredworkers}\poolUnhiredUseful{\askill}, \askill\in\task{\numtasks}_\nonhiredworkers\cap\worker{r}\right\}\\
%&=\left\{(r,\askill)\St \askill\in\task{\numtasks}_\nonhiredworkers, r\in\{r\in\poolUnhiredUseful{\askill}\St \askill\in\worker{r}\}\right\}\\
%&=\left\{(r,\askill)\St \askill\in\task{\numtasks}_\nonhiredworkers, r\in\poolUnhiredUseful{\askill}\right\},
%\end{split}\]
%where the last step follows from the fact that
%\[\poolUnhiredUseful{\askill}\subset\{r\St\askill\in\worker{r}\}.\]

Let us now consider a particular increase
$\chi_{r,\askill}^i$ of $\tilde{x}_r$ and
$\phi_{rT,\askill}^i$ of $\tilde{f}_{rT}$. Assume that the corresponding values
before the increase were
$\tilde{x}_r^{\text{old}}$ and $\tilde{f}_{rT}^{\text{old}}$.

Then we have that
\[\begin{split}
\chi_{r,\askill}^i
&=\tilde{x}_r^{\text{old}}\left(1+\frac{1}{\hiringcost{r}}\right)+\frac{1}{\numworkers\hiringcost{r}}-
\tilde{x}_r^{\text{old}}\\
&=\frac{1}{\hiringcost{r}}\cdot\left(\tilde{x}_r^{\text{old}}+\frac1n\right)
\end{split}\]
and, similarly,
\[\phi_{rT,\askill}^i=\frac{1}{\outsourcecost{r}}\cdot\left(\tilde{f}_{rT}^{\text{old}}+\frac1n\right).\]

Furthermore, because, for the increase to take place, we entered the \textbf{while} loop of step~5, we have that
\[\sum_{r\in\poolUnhired{\askill}}\left(\tilde{x}_r^{\text{old}}+\tilde{f}_{rT}^{\text{old}}\right)
=\sum_{r\in\pool{\askill}}\left(\tilde{x}_r^{\text{old}}+\tilde{f}_{rT}^{\text{old}}\right)<1.\]
(The equality is because only unhired worker possess skill~$\askill$.)

Using these two facts, we obtain that
\[
\begin{split}
\sum_{r\in\poolUnhired{\askill}}\left(\hiringcost{r}\cdot\chi_{r,\askill}^i +\outsourcecost{r}\cdot\phi_{rT,\askill}^i \right)
&=
\sum_{r\in\poolUnhired{\askill}}\left(\left(\tilde{x}_r^{\text{old}}+\frac1n\right)
+\left(\tilde{f}_{rT}^{\text{old}}+\frac1n\right)\right)\\
&<1+\frac{2\Card{\poolUnhired{\askill}}}n.
\end{split}
\]

Therefore, returning to the computation of $\E{\DeltaPrimalTimeStep{T}{8}}$, we obtain that
\begin{equation}
\label{eq:DeltaPrimal8}
\E{\DeltaPrimalTimeStep{T}{8}}
<\rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\sum_{i=1}^{\kappa_{\askill}}\left(1+\frac{2\Card{\poolUnhired{\askill}}}n\right)
\le3\rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill},
\end{equation}
using the fact that $\Card{\poolUnhired{\askill}}\le n$.

Let $\DeltaPrimalTimeStep{t}{8}$ be the increase of the objective
function incurred during the processing of task $\task{t}$ by operations
performed in step~8
%, and $\PrimalTimeStep{T}{8}$ the total cost of the objective function caused
%by operations performed in step~8.
%Analogously, let
and $\DeltaDualTime{t}$ be the cost incurred in the dual
objective function while processing task~$\task{t}$.

Combining equations~\eqref{eq:DeltaPrimal8} and \eqref{eq:DeltaDual}, we
obtain:
\begin{equation}
\label{eq:Primal8}
\frac{\E{\PrimalTimeStep{T}{8}}}{\E{\DualTime{T}}}
=\frac{\E{\sum_{t=1}^{\numtasks}\DeltaPrimalTimeStep{t}{8}}}{\E{\sum_{t=1}^{\numtasks}\DeltaDualTime{t}}}
=\frac{\sum_{t=1}^{\numtasks}\E{\DeltaPrimalTimeStep{t}{8}}}{\sum_{t=1}^{\numtasks}\E{\DeltaDualTime{t}}}
\stackrel{\mathclap{\textrm{(a)}}}{\le}3\rho_1,
\end{equation}
where $\textrm{(a)}$ follows by applying the following lemma.


\begin{lemma}
\label{lem:ratio_sums}
Let $n\in\mathbb{N}$, $a, b, c\in\mathbb{R}$, and for $i=1,\dots,n$, let $a_i, b_i\in\mathbb{R}$.
Assume that $a=\sum_{i=1}^n a_i$ and $b=\sum_{i=1}^n b_i$. If $a_i/b_i\le c$
then $a/b\le c$.
\end{lemma}
\begin{proof}
We have \(\displaystyle\sum_{i=1}^n a_i\le\sum_{i=1}^n c\cdot b_i=c\sum_{i=1}^n b_i\).
\end{proof}


%&\le3\rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill},
%
%
%
%\end{split}
%\end{equation}

Next we bound the total expected contribution to the objective function
of the primal incurred by operations of step~9 during the entire
execution of the algorithm. To start, consider a particular
skill~$\askill$ required for the current task~$\task{\numtasks}$.

Note that whenever during the execution of the algorithm $\tilde{x}_r$ is
increased, then---during the processing of the tasks that led to the
increase---in step~8 we attempt $\rho_1$ times to hire worker $\worker{r}$ with
probability $\Delta\tilde{x}_r$. Similarly, if during the processing of
the current task~\task{\numtasks} the variable
$\tilde{f}_{rT}$ became nonzero, then 
in step~8 we attempt $\rho_1$ times to outsource worker $\worker{r}$ with
probability $\tilde{f}_{r\numtasks}$.

Therefore, the probability that a worker is hired at step~9 for
skill~$\askill$ during processing of task $\task{\numtasks}$ is
bounded by the probability that none of the workers that possess the
skill was hired during the entire execution of the algorithm until (and
including) task $\task{\numtasks}$ and that no worker that possesses skill
$\askill$ was outsourced during the processing of $\task{\numtasks}$.
This probability is equal to
\[\prod_{r\in\poolUnhired{\askill}}(1-\tilde{f}_{rT})^{\rho_1}\prod_{i=1}^{\nu_r}(1-\Delta\tilde{x}_r^i)^{\rho_1}.\]
Using the fact that $1-x\le \exp(-x)$ we bound this probability by
\[\begin{split}
\prod_{r\in\poolUnhired{\askill}}&\exp(-\rho_1 \tilde{f}_{rT})\prod_{i=1}^{\nu_r}\exp(-\rho_1\Delta\tilde{x}_r^i)\\
&=\exp\left(-\rho_1\sum_{r\in\poolUnhired{\askill}}\left(\sum_{i=1}^{\nu_r}\Delta\tilde{x}_r^i+\tilde{f}_{rT}\right)\right)\\
&\stackrel{\eqref{eq:xr}}{=}
\exp\left(-\rho_1\sum_{r\in\poolUnhired{\askill}}(\tilde{x}_r+\tilde{f}_{rT})\right)\\
&\le e^{-\rho_1}=\frac1{\numskills\maxhiringcost{r}},
\end{split}\]
because, after we exited the \textbf{while} loop in step~5, we had
\[\sum_{r\in\poolUnhired{\askill}}(\tilde{x}_r+\tilde{f}_{rT})=
\sum_{r\in\pool{\askill}}(\tilde{x}_r+\tilde{f}_{rT})\ge1.\]

Note that step~9 can be executed at most $\numskills$ times: a worker
is hired only if he covers at least one new skill, after which the skill
is covered for the rest of tasks. Because the cost to
hire a new worker is at most $\maxhiringcost{r}$, we deduce that
the total expected cost of step~9 during the execution of
the algorithm is
%Therefore, the expected cost of step~9 is bounded by
\begin{equation}
\label{eq:Primal9}
\E{\DeltaPrimalStep{\PrimalTimeStep{T}{9}}}
\le1.
%\le\frac1{\numskills\maxhiringcost{r}}\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\min_{r\in\poolUnhired{\askill}}\hiringcost{r}\le1,
\end{equation}


%We conclude, as before, that the total expected cost is at most
%\begin{equation}
%\label{eq:Primal10}
%\E{\PrimalTimeStep{T}{10}}
%\le1.
%%\le\frac1{m\maxhiringcost{r}}\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\min_{r\in\poolUnhired{\askill}}\outsourcecost{r}\le1.
%\end{equation}
%
%
%
%
%
%Therefore,
%the probability that a worker is hired at step~9 for skill~$\askill$ is
%bounded by the probability that none of the workers that possess the
%skill was hired during the entire execution of the algorithm. This
%probability is equal to
%\[\prod_{r\in\poolUnhired{\askill}}\prod_{i=1}^{\nu_r}(1-\Delta\tilde{x}_r^i)^{\rho_1}.\]
%Using the fact that $1-x\le \exp(-x)$ we bound this probability by
%\[\begin{split}
%\prod_{r\in\poolUnhired{\askill}}\prod_{i=1}^{\nu_r}\exp(-\rho_1\Delta\tilde{x}_r^i)
%&=\exp\left(-\rho_1\sum_{r\in\poolUnhired{\askill}}\sum_{i=1}^{\nu_r}\Delta\tilde{x}_r^i\right)\\
%&\stackrel{\mathclap{\eqref{eq:xr}}}{=}
%\exp\left(-\rho_1\sum_{r\in\poolUnhired{\askill}} \tilde{x}_r\right)\\
%&\le e^{-\rho_1}=\frac1{\numskills\maxhiringcost{r}},
%\end{split}\]
%for $\rho_1=\ln\numskills+\ln\maxhiringcost{r}$,
%using the fact that the \textbf{if} clause of step~9 is true only when
%\[\sum_{r\in\poolUnhired{\askill}}\tilde{x}_r=\sum_{r\in\pool{\askill}}\tilde{x}_r\ge1.\]
%
%Note that step~$9$ can be executed at most $\numskills$ times: a worker
%is hired only if he coveres at least one new skill. Because the cost to
%hire a new worker is at most $\maxhiringcost{r}$, we deduce that
%the total expected cost of step~10 during the execution of
%the algorithm is
%%Therefore, the expected cost of step~9 is bounded by
%\begin{equation}
%\label{eq:Primal9}
%\E{\DeltaPrimalStep{9}}
%\le1.
%%\le\frac1{\numskills\maxhiringcost{r}}\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\min_{r\in\poolUnhired{\askill}}\hiringcost{r}\le1,
%\end{equation}
%%because $\Card{\task{\numtasks}_\nonhiredworkers}\le\numskills$.

Combining equations
\eqref{eq:Primal8} and
\eqref{eq:Primal9}
we finally obtain that
\[\E{\PrimalTime{T}}=\E{\PrimalTimeStep{T}{8}}+\E{\PrimalTimeStep{T}{9}}\le3\rho_1\cdot\E{\DualTime{T}}+1.\]
%
%\eqref{eq:DeltaDual}, 
%%\eqref{eq:DeltaPrimal5},
%\eqref{eq:DeltaPrimal8},
%\eqref{eq:DeltaPrimal9}, and \eqref{eq:DeltaPrimal10},
%we obtain that
%\[\begin{split}
%\frac{\E{\DeltaPrimalTime{T}}}{\E{\DeltaDualTime{T}}}
%%&=\frac{\sum_{i\in\{5,8,9,10\}}\E{\DeltaPrimalTimeStep{T}{i}}}{\E{\DeltaDualTime{T}}}\\
%&=\frac{
%%\E{\DeltaPrimalTimeStep{T}{5}}+
%\E{\DeltaPrimalTimeStep{T}{8}}+
%\E{\DeltaPrimalTimeStep{T}{9}}+
%\E{\DeltaPrimalTimeStep{T}{10}}}{\E{\DeltaDualTime{T}}}\\
%%&\le\frac{3\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill}+
%&\le\frac{3\rho_1\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill}+1+1}{\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill}}\\
%&\le4\rho_1,
%\end{split}\]
%\aris{
%assuming that
%$\sum_{\askill\in\task{\numtasks}_\nonhiredworkers}\kappa_{\askill}\ge1$.
%}
%\note[Aris]{Oops, why is this true?}
%
%Let $\DeltaPrimalTime{t}$ and $\DeltaDualTime{t}$ be the change incurred
%in the value of the objective values of the primal and the dual,
%respectively, objective functions, while processing task~$\task{t}$.
%By applying the same arguments that we used for task~$\task{\numtasks}$
%also to tasks $\task{t}$ for $t=1,\dots,\numtasks-1$ we have that for
%each $t=1,\dots,\numtasks$, we have
%\[\frac{\E{\DeltaPrimalTime{t}}}{\E{\DeltaDualTime{t}}}\le4\rho_1.\]
%
%Thus, finally we have
%%\[
%%\frac{\E{\Primal}}{\E{\Dual}}
%%=\frac{\E{\sum_{t=1}^{\numtasks}\DeltaPrimalTime{t}}}{\E{\sum_{t=1}^{\numtasks}\DeltaDualTime{t}}}
%%=\frac{\sum_{t=1}^{\numtasks}\E{\DeltaPrimalTime{t}}}{\sum_{t=1}^{\numtasks}\E{\DeltaDualTime{t}}}
%%\stackrel{\mathclap{\textrm{(a)}}}{\le}4\rho_1,
%%\]
%%where $\textrm{(a)}$ follows by applying the following lemma.
%%
%%
%%\begin{lemma}
%%\label{lem:ratio_sums}
%%Let $n\in\mathbb{N}$, $a, b, c\in\mathbb{R}$, and for $i=1,\dots,n$, let $a_i, b_i\in\mathbb{R}$.
%%Assume that $a=\sum_{i=1}^n a_i$ and $b=\sum_{i=1}^n b_i$. If $a_i/b_i\le c$
%%then $a/b\le c$.
%%\end{lemma}
%%\begin{proof}
%%We have \(\displaystyle\sum_{i=1}^n a_i\le\sum_{i=1}^n c\cdot b_i=c\sum_{i=1}^n b_i\).
%%\end{proof}

\spara{Analysis of feasibility of the dual LP:}
Now we show that the dual constraints are violated by a factor of at
most $2\log\numworkers$, following the approach of~\cite{buchbinder2009design}.
Similarly to~\cite{buchbinder2009design} (or proven easily by
induction), $\tilde{x}_r$ is a geometric series
whose first element is $1/\numworkers\hiringcost{r}$ with ratio
$(1+1/\hiringcost{r})$. Therefore, for any $\tau$, after $\tau$ updates we have
\[\tilde{x}_r=\frac{1}{\numworkers\hiringcost{r}}\cdot\frac{\left(1+\frac1{\hiringcost{r}}\right)^\tau-1}{\left(1+\frac1{\hiringcost{r}}\right)-1}
=\frac{\left(1+\frac1{\hiringcost{r}}\right)^\tau-1}\numworkers.\]
For $\hiringcost{r}\ge1$\footnote{Without loss of generality we can
assume that for each worker $\worker{r}$ we have $\hiringcost{r}\ge1$
and $\outsourcecost{r}\ge1$ by rescaling the costs before executing our
algorithm.} we have that
$\left(1+\frac1{\hiringcost{r}}\right)^{\hiringcost{r}}\ge2$.
Therefore, setting $\tau=2\hiringcost{r}\log \numworkers$, we have that, after $\tau$
updates, $\tilde{x}_r$ becomes at least
\[\frac{2^{2\log \numworkers}-1}\numworkers\ge 1.\]

Consider now the family of constraints~\eqref{eq:skirental-buy}. Such a
constraint
may become violated because of the increase of variables $u_{\askill t}$.
A variable $u_{\askill t}$ increases (by~1) only in step~5 of our algorithm and
only when skill $\askill$ is not covered by hired workers.
Furthermore, whenever it increases, the variables $\tilde{x}_r$ of all the
(unhired) workers who possess skill $\askill$ are updated. In the
previous paragraph we showed that after at most $2\hiringcost{r}\log
\numworkers$ updates the
value of $x_r$ becomes~1. After this takes place,
in the current and any subsequent task
the \textbf{while} statement of step~5 will evaluate to false for any
skill pocessed by worker $\worker{r}$ and the dual variable
$u_{\askill t}$ will not increase any more for $t\ge\numtasks$.
%Therefore, $u_{\askill t}$ increases by~1 at most
%$2\min_{r\in\poolUnhired{\askill}}\hiringcost{r}\log \numworkers$ times therefore we have
%that
%Note that this is true for all skills $\askill\in\worker{r}$. In other
%words, if $\tilde{x}_r$ has increased
%$2\min_{r\in\poolUnhired{\askill}}\hiringcost{r}\log \numworkers$
%times, whenever a skill $\askill\in\worker{r}$ is needed, it will either
%have already been covered by a hired worker (either $\worker{r}$ or some
%either worker) or if not yet, the \textbf{while} statement of step~5 will
%not be executed and the variable $u_{\askill t}$ will not increase any
%more.

The conclusion is that, if we look at a worker $\worker{r}$ with
$r\in\poolUnhired{\askill}$, after at most
$2\hiringcost{r}\log \numworkers$
increases of $\tilde{x}_r$, \emph{all the skills} possessed by worker
$\worker{r}$ are covered (either by worker~$\worker{r}$ or by other
workers), and $u_{\askill t}$ will not increase any more
for any $\askill\in\worker{r}$. Therefore,
\[\sum_{t=1}^\numtasks\sum_{\askill\in \task{t} \cap \worker{r}} u_{\askill
  t}\le2\hiringcost{r}\log\numworkers,\]
which means that each constraint in~\eqref{eq:skirental-buy} is
violated by a factor of at most $2\log n$.

The proof for the family of constraints~\eqref{eq:skirental-rent} is
similar: For a given task $\task{t}$ and for a given skill $\askill$, after
$u_{\askill t}$ has been increased at most
$2\outsourcecost{r}\log \numworkers$
times, $\tilde{f}_{rt}$ becomes at least 1 (assuming that
$\outsourcecost{r}\ge1$); then we exit the \textbf{while} loop
of step~5 and the variable $u_{\askill t}$ is not increased any more (for
task $\task{t}$). This implies that also the constraints in the
family~\eqref{eq:skirental-rent} are violated by a factor of at most
$2\log \numworkers$.
\end{proof}

